Scalable Graph Neural Networks via Bidirectional Propagation

Graph Neural Networks (GNN) is an emerging field for learning on non-Euclidean data. Recently, there has been increased interest in designing GNN that scales to large graphs. Most existing methods use "graph sampling" or "layer-wise sampling" techniques to reduce training time. However, these methods still suffer from degrading performance and scalability problems when applying to graphs with billions of edges. This paper presents GBP, a scalable GNN that utilizes a localized bidirectional propagation process from both the feature vectors and the training/testing nodes. Theoretical analysis shows that GBP is the first method that achieves sub-linear time complexity for both the precomputation and the training phases. An extensive empirical study demonstrates that GBP achieves state-of-the-art performance with significantly less training/testing time. Most notably, GBP can deliver superior performance on a graph with over 60 million nodes and 1.8 billion edges in less than half an hour on a single machine. The codes of GBP can be found at https://github.com/chennnM/GBP .

==> impact.tex <==
example-1:
This work has the following two potential positive impacts on society.
First, despite pre-trained language models such as BERT have achieved appealing performance in a wide range of natural language processing tasks, they are computationally expensive to be deployed in real-time applications. The proposed method can help to distill the large pre-trained models into small and effective student models for real-time resource-constrained applications, e.g. mobile applications and edge computing tasks. Second, a recent study~\cite{strubell-etal-2019-energy} shows pre-training large language models require exceptionally large computational resources that consume substantial energy. To deploy such models online is both financially and environmentally costly. Our method aims to build small and effective models to learn from the pre-trained models to save such costs for downstream applications. Our study seeks to promote research of more computationally efficient algorithms.

At the same time, this work may have one potential negative consequence. From the theoretical perspective, the proposed method is general that can be applied to distill large pre-trained language models such as GPT-3, which may enable more lightweight applications such as fake news generation on the fly. However, it is still a non-trivial task to examine the generalization capability of the proposed method for 
such applications.

example-2
The proposed HPM scheduling algorithm addresses the challenge of combining local gradient and global search for solving the hyperparameter optimization problem. The proposed framework could be incorporated in many automated machine learning systems to provide an effective hyperparameter schedule solution. The outcome of this work will benefit both the academic and industry communities by liberating researchers from the tedious hyperparameter tuning work. 
